FLuID: Mitigating Stragglers in Federated Learning using Invariant Dropout

Federated Learning (FL) allows machine learning models to train locally on individual mobile devices, synchronizing model updates via a shared server. This approach safeguards user privacy; however, it also generates a heterogeneous training environment due to the varying performance capabilities across devices. As a result, straggler devices with lower performance often dictate the overall training time in FL. In this work, we aim to alleviate this performance bottleneck due to stragglers by dynamically balancing the training load across the system. We introduce Invariant Dropout, a method that extracts a sub-model based on the weight update threshold, thereby minimizing potential impacts on accuracy. Building on this dropout technique, we develop an adaptive training framework, Federated Learning using Invariant Dropout (FLuID). FLuID offers a lightweight sub-model extraction to regulate computational intensity, thereby reducing the load on straggler devices without affecting model quality. Our method leverages neuron updates from non-straggler devices to construct a tailored sub-model for each straggler based on client performance profiling. Furthermore, FLuID can dynamically adapt to changes in stragglers as runtime conditions shift. We evaluate FLuID using five real-world mobile clients. The evaluations show that Invariant Dropout maintains baseline model efficiency while alleviating the performance bottleneck of stragglers through a dynamic, runtime approach.

==> body/proof.tex <==
\section{Convergence of Invariant Dropout}
% CD dropout is a set of of FL that has N clients and a percentage of slower clients receive a subset of the global model, while the majority of clients still train on the full global model. 

% Gradient Sparsification for Communication-Efficient Distributed Optimization: 
%https://proceedings.neurips.cc/paper/2018/file/3328bdf9a4b9504b9398284244fe97c2-Paper.pdf

% prior work [] has already proved that the variance of gradients across neurons will significantly affect the convergence efficiency of the global model. As well, the work has shown that a sparse gradient with top- K largest magnitude of gradient variance is bounded hence will converge.  
% CD dropout uses an threshold to approximate the set of neurons withe the largest gradient variance

% The majority of clients still train on the full model, while a smaller percentage of straggler  train on the subset of neurons with larger magnitude of gradient variance. Therefore the model convergences with CD dropout? 
%Locally optimizer: FEMNIST: SGD, CIFAR10: Adam, and Shakespeare: ADAM
%Server side : SGD (vanilla FedAvg) 

%The server side update:
%$\Theta_{t+1} = \frac{1}^{N}\sum_{i=1}^{N} \Theta_{t}^{i}$
%
%Let $\Delta^t_i := x^t_i - x_t$, and $\Delta^t := \frac{1}{N}\sum_{i=1}^{N} \Delta^t_i$. The server update in FedAvg algorithms is equivalent to applying SGD with a gradient of "$-\delta_t$, with a learning rate of $\eta =1$. ~\cite{reddi2021adaptive}
%
%Hence our technique still uses the same SGD optimizer on server size: 

Similar to the prior work~\cite{GradientSF}, although dropout can reduce the communication cost of stragglers but can increase the gradient variance.
%
We prove convergence of our invariant dropout technique using bounded gradient variance~\cite{GradientSF, helios}.
%
Consider $N$ devices participating in Federated Learning. 
%
The training data is represented as $\{x_{n}\}_{n=1}^{N}$, where $n$ represents a device, and each one has a loss function $\{f_{n}\}_{n=1}^{N}$.
%
We solve to the minimize the loss function using the following optimization: 


\begin{equation}
    f(w) := \frac{1}{N} \sum_{n=1}^{N} f_n(w)
\end{equation}

\begin{equation}
    w_{t+1} = w_{t} - \eta_t(g(w_t))
\end{equation}

The invariant dropout problem can be viewed as a sparse stochastic gradient vector, where each gradient has a certain probability to be dropped. 
%
The gradient vector is $G = [g_1, g_2, ...,  g_m]$ where $g \in R$ with probability of staying and being transmitted across the networks as $[p_1, p_2, ...,  p_m]$.
%
Hence, the probability of dropout is $1 - p_i$, where $0 < i \le m$.
%
The sparse vector for the stragglers is represented as $G_s$.
%
The variance of the invariant-dropout based gradient vector can be represented as follows: 

\begin{equation}
    E\sum_{i=1}^{m}[(G_s)]^2 = \sum_{i=1}^{m} (\frac{g_i^2}{p_i})
\end{equation}

The variance of the dropout vector is a small factor deviation from the non-dropout gradient vector represented as follows: 

\begin{equation}
   \min \sum_{i=1}^{m} p_i : \sum_{i=1}^{m} (\frac{g_i^2}{p_i}) = (1 + \epsilon) \sum_{i=1}^{m}{g_i^2}
   \label{eq:variancesparisityoptimization}
\end{equation}

This aims to minimize the probability of selecting gradients, i.e. higher benefits from skipping gradients, whilst ensuring the variance being small deviation from the dense gradient vector. 

\subsubsection{Proof of convergence:}
%
With the invariant dropout, the weights are dropped based on their `percentage' change across iterations which essentially implies that weights corresponding to higher gradient values have a lower probability of being dropped and vice-versa.
%
This implies if $|g_i > g_j|$ then $p_i > p_j$.
%
The probability of a gradient getting dropped is proportional to the invariant dropout rate $r$.
%
Lets assume, in this case the top-k magnitude of gradient values are not dropped, hence if $G = [g_1, g_2, ...,  g_m]$ is assumed to be sorted, then $G = [g_1, g_2, ...,  g_k]$ has a $p = 1$, whereas the $G = [g_{k+1}, g_{k+2}, ...,  g_d]$ have a probability of $p_i = r|g_i|$.
%
This modifies the optimization problem in Equation~\ref{eq:variancesparisityoptimization} to the following: 

\begin{equation}
    \sum_{i=1}^{k} {g_i^2} + \sum_{i=k+1}^{m} \frac{|g_i|}{r} - (1 + \epsilon) \sum_{i=1}^{m}{g_i^2} = 0, r|g_i| \leq 1
\end{equation}

Which implies that

\begin{equation}
    r = \frac{\sum_{i=k+1}^{m} |g_i|}{(1 + \epsilon) \sum_{i=1}^{m}{g_i^2} - \sum_{i=1}^{k} {g_i^2}}
\end{equation}

As per the constraint $r|g_i| \leq 1$:

\begin{equation}
    |g_i|(\sum_{i=k+1}^{m} |g_i|) \leq (1 + \epsilon) \sum_{i=1}^{m}{g_i^2} - \sum_{i=1}^{k} {g_i^2}
\end{equation}

In this invariant dropout work we keep the gradients with highest magnitude, thus if the number of gradients. As per~\cite{GradientSF}, if $k << d$ the boundedness of the expected value from equation~\ref{eq:variancesparisityoptimization} can be represented as:

\begin{equation}
   \sum_{i=1}^{m} p_i, = \sum_{i=1}^{k} p_i + \sum_{i=k+1}^{m} p_i
\end{equation}

\begin{equation}
   \sum_{i=1}^{m} p_i = k + |g_i| \sum_{i=k+1}^{m} (\frac{\sum_{i=k+1}^{m} |g_i|}{(1 + \epsilon) \sum_{i=1}^{m}{g_i^2} - \sum_{i=1}^{k} {g_i^2}})
\end{equation}

\begin{equation}
   \sum_{i=1}^{m} p_i \leq k(1 + \epsilon)
   \label{eq:boundedness}
\end{equation}

This proves that the variance of gradient is bounded by Equation~\ref{eq:boundedness}.
